ReMatch: Retrieval Enhanced Schema Matching with LLMs

Schema matching is a crucial task in data integration, involving the alignment of a source schema with a target schema to establish correspondence between their elements. This task is challenging due to textual and semantic heterogeneity, as well as differences in schema sizes. Although machine-learning-based solutions have been explored in numerous studies, they often suffer from low accuracy, require manual mapping of the schemas for model training, or need access to source schema data which might be unavailable due to privacy concerns. In this paper we present a novel method, named ReMatch, for matching schemas using retrieval-enhanced Large Language Models (LLMs). Our method avoids the need for predefined mapping, any model training, or access to data in the source database. Our experimental results on large real-world schemas demonstrate that ReMatch is an effective matcher. By eliminating the requirement for training data, ReMatch becomes a viable solution for real-world scenarios.

==> Sections/5-Related-Work.tex <==
\section{Related Work}
\label{sec:related_work}

Prior work has dealt with various ML based matchers to tackle the schema matching task, but these have often resulted in low-quality matches or necessitated extensive manual annotation~\cite{Bernstein2011GenericSM}. 

More recent mechanisms often employed similarity matrices between schemas, with various ML or deep learning (DL) components~\cite{Mudgal2018DeepLF,Shraga2020ADnEVCS, Li2020DeepEM}, but these were limited to small datasets, like Purchase Orders~\cite{Do2002COMAA}, or Web Forms~\cite{Gal2011UncertainSM}, and focused primarily on entity matching rather than schema matching. More recent work in the field such as SMAT~\cite{Zhang2021SMATAA} and LSM~\cite{Zhang2023SchemaMU} has been proposed, leveraging recent improvements in natural language processing techniques to obtain semantic mappings between source and target schemas. These approaches improved previous results, but still demanded that a large percentage of the data be tagged, making real-world usage impractical. 

LLMs have been applied to various data preprocessing tasks, including error detection, data imputation, entity matching, as well as schema matching~\cite{Mirchandani2023LargeLM, Narayan2022CanFM}. These models have shown promising results, with LLMs achieving good results on various datasets, with no additional training involved. However, these approaches still faced challenges related to computational expense and inefficiency, as well as lacking evaluation on data that represents real-world schema matching challenges. 

Finally, it is important to note that the majority of previous methods dealt with schema-matching as a binary classification task over the full Cartesian-product $\mathcal{A}_1 \times \mathcal{A}_2$. While allowing for simplified training objectives and evaluations, in normalized schemas positive labels scale by $O(n)$, whereas negative labels scale by $O(n^2)$. This is especially problematic when inference is expensive, as in the case of LLMs. 
